Predict Responsibly: Improving Fairness and Accuracy by Learning to Defer

In many machine learning applications, there are multiple decision-makers involved, both automated and human. The interaction between these agents often goes unaddressed in algorithmic development. In this work, we explore a simple version of this interaction with a two-stage framework containing an automated model and an external decision-maker. The model can choose to say "Pass", and pass the decision downstream, as explored in rejection learning. We extend this concept by proposing "learning to defer", which generalizes rejection learning by considering the effect of other agents in the decision-making process. We propose a learning algorithm which accounts for potential biases held by external decision-makers in a system. Experiments demonstrate that learning to defer can make systems not only more accurate but also less biased. Even when working with inconsistent or biased users, we show that deferring models still greatly improve the accuracy and/or fairness of the entire system.

==> paper-body.tex <==
\section{Introduction}
Recent advances in the accuracy of machine learning algorithms have drastically increased
our reliance on learned automated systems to make complex decisions. Our trust in these systems
is a cause for concern, particularly in life-altering domains such as
loan approvals \citep{burrell2016machine},
%[19],
medical diagnosis \citep{esteva2017dermatologist}, or
criminal justice \citep{kirchner_machine_2016}.

This growing use of
automated decision-making systems has raised questions
about unfairness in classification systems, and
sparked much debate and discussion among philosophers, policy-makers, lawyers
and computer scientists.
For example, risk assessments are increasingly common
in courtrooms \citep{hannah2013actuarial}, where they are used to help make decisions at various
levels, from assigning bail amounts to criminal sentencing.
One highly publicized case involves the proprietary COMPAS system 
\cite{compas_2012},
an algorithm used for risk assessment and the prediction of
recidivism in the United States.
It was found that the COMPAS algorithm
made disproportionately more false positive errors (predicting high risk for
individuals who did not recidivate) for black people than for white people \cite{kirchner_machine_2016,liptak_nyt_2017,kirchner_2016}.
Other reports have revealed similar biases in the New York Police Department's
stop-and-frisk program \cite{goel_2016} and targeted advertising \cite{sweeney_2013}.


%(e.g., \cite{dwork_fairness_2011,kleinberg_inherent_2016,zemel_learning_2013,kusner_counterfactual_2017,hardt_equality_2016,zafar_fairness_2017,grgic_hlaca_fairness_2017,bechavod_learning_2017,bower_fair_2017,kilbertus_avoiding_2017,jabbari_fairness_2016}.)
%The two most well-studied notions of fairness are
%disparate impact and disparate ??.

In this paper we will use {\it disparate} {\it impact} as
a measure of fairness. 
Disparate impact is well-established within the legal system \citep{rutherglen1987disparate}, and has been
proposed as a measure of fairness for supervised learning tasks in several recent papers 
\cite{kleinberg_inherent_2016,hardt_equality_2016,zafar_fairness_2017}.
Minimized disparate impact (also called equalized odds) maintains that the accuracy (false positive
and false negative rates) of the learning
algorithm should be the same across all demographics.
While not solving all of the possible sources of unfairness,
disparate impact is a clear fairness goal.
%The one-sided version (called {\it equal opportunity}), where the false negative rates
%are equal across all groups (and where positive is the
%desired outcome) was also studied \cite{hardt-price-srebro}.

Unfortunately, 
no well-calibrated classification system (where calibration measures accuracy conditioned on the true outcome)
can minimize disparate impact \cite{kleinberg_inherent_2016,chouldechova_fair_2016}.
Given this incompatibility,
previous papers have either weakened the fairness requirements,
or have suffered a loss in one or both of these goals.
This leaves us in a no-win situation: either we relax fairness criteria
(leaving the classification algorithm unfair)
or we inevitably need to reverse some
well-calibrated examples.

%Furthermore, many of these models are bad at estimating
%their own uncertainty, and this is excaserbated by the fact that
%the models can be quite non-transparent.
%especially the highest accuracy ones, which
%People can over-trust models ("the algorithm made me do it")
%When should we trust an algorithm and when should
%human experts override its decision?

Given that achieving both accuracy and fairness on the full dataset is not attainable, we propose an alternative: allowing the automated system to not produce a classification decision on every example.
That is, the learning algorithm can
\textit{defer} the classification decision on some data.
When deferring, the algorithm does not output a prediction; rather it says ``I don't know'' (IDK), indicating it has insufficient information to make a reliable prediction. We see three advantages in this approach. Firstly, we hypothesize that an IDK option can help learning algorithms for classifiers to maintain both accuracy and fairness by deferring on difficult examples. Furthermore, we assert that algorithms which can declare uncertainty are more transparent, allowing for better user interaction and explainability. Finally, we believe that algorithms which can defer, i.e. yield to more informed decision-makers when they cannot predict responsibly, are an essential component to making automated systems more accountable and reliable.

We view learning to defer
as a design decision
and a key gain over previous work.
Our view is that any classification algorithm for a complex task should be understood
as one of many components within a pipeline, and that the goal of each component is to be
as accurate and fair as is possible given the resources and information
available. Particularly in complex domains, the algorithm should be aware that
they are not always in a position to decide, and that further investigation may be required.
Deferred cases would therefore be moved
downstream where a more informed decision can be made.
For example, in medical diagnosis, the deferred cases would
lead to more medical tests, and a second expert opinion.
In the case of an admissions or loan decision, the deferred cases
would be flagged and sent to a committee for further discussion.
%Last scenario: judges with risk scores

Incorporating a deferral option into machine learning algorithms
aligns with the philosophy of \cite{dwork_fairness_2011,raw_2001}, that fairness should
be as transparent as possible, subject to debate and open to the public.
It also supports the viewpoint articulated in \cite{grgic_hlaca_fairness_2017}
that in order to maintain diversity,
automated classification algorithms should be designed to work in cooperation
with a variety of decision makers, rather than to replace them.

In this paper we propose machine learning models that attempt to optimize both accuracy and fairness, while also communicating their own uncertainty.
We propose different formulations of these models and explore the
trade-offs, on two real-world datasets, from the legal and health domains.
Our first primary finding is that introducing an IDK response allows the model to improve the combination of accuracy and disparate impact beyond the effects of simple regularization.

Our second primary finding is that when the learning model has insight into decision makers later in the pipeline, it can leverage this information to improve the accuracy and disparate impact of the \textit{pipeline as a whole}.
We simulate such a pipeline where our model can defer judgment to a downstream decision maker who is sometimes more informed, echoing real-world situations where decision makers later in the chain have more resources or information for economic, security or contextual reasons.
%the interplay between a model that can say IDK and a simulated human user
We propose a learning algorithm for training a model that can work optimally \textit{with} such a decision-maker,
by learning where the user knows things that the model doesn't. Our experimental results demonstrate that this algorithm can help us to learn systems which, through expressing their uncertainty, can work with users to make fairer, more transparent decisions.


% Considering the possibility of a DM with higher accuracy is important for several reasons. Algorithms operate in many complex scenarios today, where expert opinion is necessary, or where not all information can either be made available or effectively digitized. For instance, it is possible that the DM has access to some sensitive information, which cannot be exposed to the algorithm for privacy/security reasons. There may be qualitative or highly complex variables at play, such as spoken testimony or a written report. The DM may be a computationally intensive model, which has access to technical resources that the IDK model does not. Therefore, we think the situation of a more accurate DM is a very valuable one to explore. Our results, which suggest that a simple model with the capacity to say IDK can improve the fairness of systems which rely on these DMs, are therefore highly relevant to a wide variety of applications.



\section{Related Work}

\noindent{\bf Notions of Fairness.}
Recently, there has been a significant amount of work surrounding the question of fairness in machine learning. 
% Fairness is a complex and multi-faceted problem; many 
% potential sources of unfairness exist, and the subtleties of the problem
% have been well-articulated 
% (e.g., \cite{dwork_fairness_2011,moritz_unfair_blog,moritz_unfair_blog2}).
Several works have focused on the goal of treating similar people similarly (individual fairness)
and the resulting necessity of fair-awareness  --
showing that it may be essential to give the algorithm knowledge of the sensitive variable \cite{dwork_fairness_2011,zemel_learning_2013,dwork_decoupled_2017}. 
Recent causal approaches have been taken to fairness e.g. \cite{kusner_counterfactual_2017,kilbertus_avoiding_2017};
 however we will not address this aspect of the literature in this work. 
Some fairness approaches that use neural networks, as we do, include \cite{louizos_variational_2015,edwards_censoring_2015} - however, these focus on generative models, whereas we work with exclusively discriminative learning. 

Some definitions of fairness center around the idea 
of statistical parity (e.g.,\cite{kamiran_classifying_2009,kamishima2012fairness}), or calibration (e.g., \cite{pleiss_fairness_2017,guo_calibration_2017}) or
disparate impact/equalized odds \cite{chouldechova_fair_2016,hardt_equality_2016,kleinberg_inherent_2016,zafar_fairness_2017}.
Since we use disparate impact as our measure of fairness, we focus our discussion of related
works on this measure.

\cite{hardt_equality_2016} present two notions of disparate impact,
``equal opportunity'' which requires equal false negative as well as false positive
rates on each of the groups, and ``equalized odds'' that only requires
that false negative rates are equal. They propose an elegant post-processing algorithm
to correct an unfair trained classifier, and prove that it is
Bayes optimal. 
% Their algorithms are easy to implement, and can be used with any existing classifier.
In a subsequent paper, \cite{woodworth_learning_2017} argue that the post-hoc approach in practice can give
a sub-optimal classifier and suggest that
in practice fairness criteria should be part of
the learning algorithm.
They propose a two-step learning process
where the first step trains with a discriminatory constraint,
followed by a further post-training step, with provably good
generalization. Unfortunately the procedure is computationally
intractable, and while they propose relaxed versions,
it is not clear how well they perform.
\cite{zafar_fairness_2017,bechavod_learning_2017} develop and implement
learning algorithms that integrate equalized
odds into learning via regularization. Both of these works
are implemented on the COMPAS dataset (as well as on other datasets).

As mentioned in the introduction, it was shown 
that disparate impact as well as calibration 
cannot be simultaneously satisfied \cite{chouldechova_fair_2016,kleinberg_inherent_2016}.
\cite{kleinberg_inherent_2016} present a much more general setup where accuracy
and disparate impact are incompatable; \cite{chouldechova_fair_2016} gives the
same basic result, including a beautifully simple explanation (see top of p.3)
for the incompatability of these concepts. 

\noindent{\bf Incorporating IDK.}
Some works have examined the idea of using an IDK option. 
There is a fairly large body of literature of IDK in the form of confidence-based rejection,
beginning with the work of Chow \cite{chow_1957,chow_1970}who studied the tradeoff between error-rate and rejection rate,
and gave an analysis of the Bayes optimal decision for this setting.
%(TONI COMMENT: similar to what Hardt paper does post-hoc for fairness.)
Subsequent works include \cite{bartlett_wegkamp_2008}; see \cite{cortes2016learning}
for a thorough survey of previous work.)
\cite{cortes2016learning} were the first to develop a framework
for integrating IDK directly into learning. They give a theoretical
analysis of their framework, and using kernel-based algorithms,
they demonstrate empirical gain on some datasets.

KWIK (Knows-What-It-Knows) learning is proposed in \cite{li_knows_2011} as a theoretical framework for saying IDK.  
\cite{wang_idk_2017} proposes a cascading model, which can be learned from end-to-end; higher levels can say IDK and pass the decision on to lower levels. Similarly, \cite{kocak_safepredict:_2017,cortes2016learning} both provide algorithms for saying IDK in classification. However, none of these works look at the fairness impact of this procedure, nor does it take into account what happens to the examples the model says IDK to. At a more general level, Bayesian learning such as \cite{blundell_weight_2015} is another method of learning uncertainty; this is not an approach we address in this work.

A few papers have approached topics which are related to both of these ideas. \cite{bower_fair_2017} describe fairness in sequential decision making - however, the pipeline they formulate does not have an IDK concept, nor do they provide a learning procedure for learning a fair pipeline. In \cite{jabbari_fairness_2016}, the authors connect KWIK-learning with a proposed method for fair reinforcement learning; however, the reinforcement learning setting is extremely different from the supervised learning setting in both theory and practice, and the paper shows no experimental results. \cite{grgic_hlaca_fairness_2017} discuss fairness that can arise out of a mixture of classifiers. However, they do not provide a procedure for learning this mixture, nor do they address the sequential decision making setting, which we believe is of great practical importance.

\noindent{\bf AI Safety.}
Finally, our work also touches on aspects of the AI safety literature - we provide a method by which a machine learns to work optimally with a human. This is conceptually similar to work such as \cite{milli_should_2017,soares2015corrigibility}, which discuss the situations in which a robot should be compliant/cooperative with a human. The idea of a machine and human jointly producing a fair classifier also relates to \cite{hadfield2016cooperative}, which describes algorithms for machines to align with human values.

Hence, our contributions are threefold: we examine the idea of an IDK option combined with fairness, we directly address the interplay of a deferring model and its surrounding system, and we provide a framework for assessing the effect of an IDK model across the entire pipeline.

\section{Fair Binary Classification} \label{binary_class}
\subsection{Accuracy vs. Fairness}
In this section, we introduce and discuss fair binary classifiers. The typical fair classification setup involves four variables: data $X$, labels $Y$, predictions $\hat{Y}$, and sensitive attribute $A$. $X$ is made up of examples $x_i \in \mathcal{R}^D$ where $D$ is the dimension of the data; often we assume for simplicity that $Y, \hat{Y}, A \in \{0, 1\}$. When we learn a classifier for $X$, the classifier outputs a prediction $\hat{Y}_i$ for each example $x_i$. The aim is twofold: firstly, that the classifier's predictions $\hat{Y}$ are \textit{accurate} i.e., $Y_i = \hat{Y}_i$ frequently; and secondly, that the classifier is \textit{fair with respect to A} i.e., the predictions $\hat{Y}$ do not discriminate unfairly against examples with a particular value of $A$.

The difficulty in learning a fair binary classifier is the trade-off between accuracy and fairness. This tradeoff is similar to the calibration-fairness tradeoff mentioned in the introduction, since accuracy and calibration are closely related; we focus on accuracy rather than calibration in this work. Intuitively, a model with fairness constraints will not be able to achieve the same error rate that it achieved without fairness constraints. In order to learn a classifier which is both accurate and fair, we define a loss function which trades off between these two objectives. This loss function relaxes the hard fairness constraint proposed by models such as \citep{hardt_equality_2016}. The loss function is defined on the label $Y$, the prediction $\hat{Y}$ and the sensitive variable $A$, which we assume to all be binary.
\begin{equation}
\begin{aligned}
\mathcal{L}(Y, A, \hat{Y}) = \mathcal{L}_{acc}(Y, A, \hat{Y}) + \alpha \mathcal{L}_{fair}(Y, A, \hat{Y})
\end{aligned}
\end{equation}

There is one term in the loss function for accuracy ($\mathcal{L}_{acc}$) and one for fairness ($\mathcal{L}_{fair}$), essentially regularizing our loss function to encourage fair solutions. This approach is similar to that taken by \citep{kamishima2012fairness,bechavod_learning_2017}.  We describe the form of these terms in section \ref{fair_learning_in_practice}. Note the hyperparameter $\alpha$, which trades off between accuracy and fairness. Since there is no ``correct'' way to balance these two objectives, the flexibility added by $\alpha$ is essential.

\subsection{Defining Fairness as Disparate Impact}
We use disparate impact as our fairness metric, formulated similarly to \citep{chouldechova_fair_2016}. Disparate impact measures the difference in effect a policy has across two groups.  We define disparate impact (DI) in terms of binary $Y, A, \hat{Y}$ as
\begin{equation} \label{discrete_di}
\centering
\begin{aligned}
DI_{Y=0}(Y, A, \hat{Y}) &= | P(\hat{Y} = 1 | A = 0, Y = 0) - P(\hat{Y} = 1 | A = 1, Y = 0) |\\
DI_{Y=1}(Y, A, \hat{Y}) &= | P(\hat{Y} = 0 | A = 0, Y = 1) - P(\hat{Y} = 0 | A = 1, Y = 1) |\\
DI(Y, A, \hat{Y}) &= \frac{1}{2} (DI_{Y=0}(Y, A, \hat{Y}) + DI_{Y=1}(Y, A, \hat{Y}))
\end{aligned}
\end{equation}
Informally, $DI_{Y=0}, DI_{Y=1}$ are the absolute difference between the two groups in false positive and false negative rates, respectively; we define DI as the mean of these two terms. Constraining that $DI = 0$ is equivalent to the constraint of equalized odds \citep{hardt_equality_2016}. It is also similar to the notion of ``balance for the positive/negative class'' raised in \citep{kleinberg_inherent_2016}, who define the metric in terms of average risk scores, whereas we work with probabilities over binary variables. In the language of \citep{chouldechova_fair_2016}, $DI_{Y=1}$ (or $DI_{Y=0}$) is the difference in average penalty of those who do (or do not) have $Y = 1$, with the high and low risk penalties set to 1 and 0, respectively.


\subsection{Learning Fairly in Practice} \label{fair_learning_in_practice}
We regularize our models with a term inspired by disparate impact, similarly to \citep{bechavod_learning_2017}. $DI$ is defined in terms of binary outputs $\hat{Y}$. However, in a logistic regression model, the classifier outputs a probability $p_i = P[Y_i = 1] \in [0, 1]$. We use these probabilities $p_i$ to define our regularization term $DI_{reg}$, a continuous relaxation of $DI$ that we can use in training. When $p \in [0, 1]$ we say we are training with \textit{soft thresholds}.

\begin{equation} \label{cont_di}
\begin{aligned}
DI_{reg,Y=0}(Y, A, p) &= | E(p_i | A = 0, Y = 0) - E(p_i | A = 1, Y = 0) |\\
DI_{reg,Y=1}(Y, A, p) &= | E(1 - p_i | A = 0, Y = 1) - E(1 - p_i| A = 1, Y = 1) |\\
DI_{reg}(Y, A, p) &= \frac{1}{2} (DI_{reg,Y=0}(Y, A, p) + DI_{reg,Y=1}(Y, A, p))
\end{aligned}
\end{equation}

Then, our regularized fair loss function 
%$\mathcal{L}_{Fair}$ or 
$\mathcal{L}_{F}$ is
\begin{equation} \label{cont_di_loss}
\begin{aligned}
\mathcal{L}_{F}(Y, A, p) = -\bigg[\sum_i Y_i \log{p_i} + (1 - Y_i) \log{(1 - p_i)}\bigg] + \alpha DI_{reg}(Y, A, p)
\end{aligned}
\end{equation}

where the first term is the negative log-likelihood of the training labels (a standard measure of accuracy), and the second term is our disparate impact regularizer, with the coefficient $\alpha$ to trade off between accuracy and fairness. Echoing \citep{bechavod_learning_2017}, we find this method to be effective in binary classifiers at reducing DI without impacting its accuracy too much. More detailed results are given in the Appendix. Note that $p$ may be constrained to be binary, ie.,  $p \in \{0, 1\}$, in which case we say we are training with \textit{hard thresholds}. Then Equations \ref{discrete_di} and \ref{cont_di} are equivalent, and we can write our loss function $\mathcal{L}_{F}^{Hard}$ as
\begin{equation} \label{cont_di_loss}
\begin{aligned}
\mathcal{L}_{F}^{H}(Y, A, p) = -\bigg[\sum_i \mathbbm{1}[Y_i == p_i]\bigg] + \alpha DI(Y, A, p); p \in \{0, 1\}
\end{aligned}
\end{equation}

\section{Learning What You Don't Know} \label{ternary_class}

\subsection{Classification with IDK Option}

In this section, we extend the binary classification model, introducing IDK as a third possible output. In binary classification, one often uses a threshold $t$ to discriminate between two groups of examples. Examples on one side of $t$ are labelled ``positive'', examples on the other side, ``negative''. For instance, in logistic regression, $t = 0$, so examples for which the model's output is greater than 0 are classified as positive; and otherwise they are classified as negative.

In this work, we propose adding a third option: a model which can classify examples as ``positive'', ``negative'' or ``IDK''. This allows the model to \textit{punt}, to output an IDK prediction when it does not want to commit to a hard positive or negative prediction. To extend the binary model, we use two thresholds: $t_0$ separates the negative examples from the IDK's, and $t_1$ separates the positive examples from the IDK's.
\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{idk_classifier_thresholds.pdf}
\caption{Binary classification (one threshold) vs. IDK classification (two thresholds)}. 
\end{figure}
In this section, we propose a model for an IDK classifier, which is based on ordinal regression. We propose two methods for learning these thresholds: an end-to-end method, and a post-hoc method. Another class of model, simply a three-way multi-class classifier, we chose not to explore, since it did not express the ordinal nature of the problem.

Previously, we mentioned that a fair binary classifier must trade off between two objectives: accuracy and fairness. A fair IDK classifier must trade off between three objectives: accuracy, fairness and uncertainty. A classifier which says IDK almost all the time is practically useless; it must learn to minimize the number of mistakes it makes, without saying IDK on too many examples.

% We take the convention of using the symbol "1" to represent a positive prediction, "0" to represent a negative prediction, and "Z" to represent an IDK prediction.

\subsection{IDK Models: Learning to Punt}
We base our IDK models on ordinal regression with three categories (positive, IDK, and negative). These models involve learning a pair of thresholds $(t_0, t_1)$. We can train with either hard or soft thresholds. If soft, each threshold $t_i$ is associated with a sigmoid function $\sigma_i$, where
\begin{equation}
\begin{aligned}
\sigma_i(x) = \sigma(x - t_i); \ \ \ \ \ \ \ \ \sigma(x) = \frac{1}{1 + e^{-x} } 
\end{aligned}
\end{equation}

These thresholds then yield an ordinal regression, which produces three numbers for every score $x_i$: $P_i, I_i, N_i \in [0, 1]$, such that $P_i + I_i + N_i = 1$. These numbers are determined by:
\begin{equation} \label{ordreg}
\begin{aligned}
P_i &= \sigma_1(x_i)\\
I_i &= \sigma_0(x_i) - \sigma_1(x_i)\\
N_i &= 1 - \sigma_0(x_i)\\
\end{aligned}
\end{equation}
We can interpret these numbers as gambles: $P$ represents the model's bet that $x$ belongs to the positive class, $N$ the bet that $x$ belongs to the negative class, and $I$ is the model hedging its bets; this bet will be higher if the model is more unsure. We can also calculate a score $p_i \in [0, 1]$, which we can interpret as the model's prediction disregarding uncertainty. Note that $p_i = 0.5$ when $P_i = N_i$, which is also when $I_i$ is maximized.
\begin{equation} \label{defn_p}
\begin{aligned}
p_i &= \frac{P_i}{P_i + N_i}\\
\end{aligned}
\end{equation}

We use a loss function for IDK models which trades off between accuracy and uncertainty. This loss function ($\mathcal{L}_{Punt}$ or $\mathcal{L}_{P}$ )is analogous to the fair binary classification loss:
\begin{equation}
\begin{aligned}
\mathcal{L}_{P}(Y, (P, N, I)) = -\bigg[\sum_i Y_i \log{P_i} + (1 - Y_i) \log{N_i} - \gamma\log{I_i}\bigg]
\end{aligned}
\end{equation}

Note that we add a term penalizing any probability mass put on $I_i$ - preventing the trivial solution of always outputting IDK. We can control how much we penalize saying IDK by increasing or decreasing $\gamma$.

At test time, we use the thresholds to partition the examples into two groups. On each example, the model outputs a score $x_i \in \mathcal{R}$ (the logit for the ordinal regression), and a prediction $p_i$ (the model's prediction, independent of uncertainty (defined in Equation \ref{defn_p})). If $t_0 < x_i < t_1$, then we replace the model's prediction $p_i$ with IDK. If $x_i \leq t_0$ or $x_i \geq t_1$, we leave the prediction $p_i$ as is, simply rounding $p_i$ to 0 or 1, whichever is closer. This produces a ternary classifier.

We propose two methods for finding these thresholds. The first is an end-to-end model, which learns the thresholds $(t_0, t_1)$ and the scores $x_i$ jointly. This model uses soft thresholds to learn. The second method is a post-hoc thresholding model, which first learns a fair binary classifier with a soft threshold (as in Equation \ref{cont_di_loss}), and then, as a second step, optimizes thresholds (either hard or soft) over top of these scores. We can use any post-hoc search procedure we like to find these thresholds.


% To find the thresholds we use a search procedure described in below. It aims to minimize the following loss function:
% \begin{equation}
% \begin{aligned}
% L = (\sum_i \mathbbm{1}[Y_i == \hat{Y}_i] + \gamma \mathbbm{1}[\hat{Y}_i == IDK]) + \alpha DI(Y, A, \hat{Y})
% \end{aligned}
% \end{equation}
% where $\gamma$ is a hyperparameter controlling how much worse we think a mistake is than saying IDK. Note that we are able to use the discrete output $\hat{Y}$ here, rather than the continuous $p$. This is because the training procedure we use for thresholding does not require differentiability.



%\subsection{End-to-end Model}

% The second model we propose is learned in one stage - the output scores and the thresholds are learned simultaneously. For this model, we use an ordinal regression on top of a one layer neural network. The ordinal regression learns the two thresholds ($t_0, t_1$), which are both represented as sigmoid functions ($\sigma_0, \sigma_1$).

% The ordinal regression produces three numbers for every score; call them $s_0, s_1, s_2$, such that $s_0 + s_1 + s_2 = 1$. The numbers are determined by:
% \begin{equation}
% \begin{aligned}
% s_2(x) &= \sigma_1(x)\\
% s_1(x) &= \sigma_0(x) - \sigma_1(x)\\
% s_0(x) &= 1 - \sigma_0(x)\\
% \end{aligned}
% \end{equation}
% We can take $s_2$ as the probability of positive, $s_0$ as the probability of negative, and $s_1$ as the probability of IDK.

% We use a loss function which trades off between accuracy, fairness, and saying IDK. This loss function is analogous to the fair binary classification loss:

% Then, our regularized loss function is
% \begin{equation}
% \begin{aligned}
% L = &(\sum_i Y_i \log{s_{2_i}} + (1 - Y_i) \log{1 - s_{0_i}} + \gamma(\log{s_{1_i}})) \\
% \end{aligned}
% \end{equation}

% Note that we've added a term penalizing any probability mass put on $s_1$.

\subsection{Learning Fairly in IDK Models}
We can modify these models to further encourage fairness. For example, we can learn a separate set of thresholds for each group, where groups are defined by the value of the sensitive variable $A$. \citep{dwork_fairness_2011,dwork_decoupled_2017} show this is a helpful and sometimes necessary step for fairness. In this case, we would learn two pairs of thresholds: $(t_{0,A=0}, t_{1,A=0})$ and $(t_{0,A=1}, t_{1,A=1})$, and simply apply the appropriate set of thresholds to each example.


% In the post-hoc method, our new loss function looks like this:
% \begin{equation}
% \begin{aligned}
% L = (\sum_i \mathbbm{1}[Y_i == \hat{Y}_i] + \gamma \mathbbm{1}[\hat{Y}_i == Z]) + \alpha DI(Y, A, \hat{Y})
% \end{aligned}
% \end{equation}
% Note again that we are able to use the discrete output $\hat{Y}$ in $DI$, rather than a continuous probability $p$.

Furthermore, we can regularize IDK classifiers for low disparate impact, in a similar way to binary classifiers. Using soft thresholds, the regularized loss function $\mathcal{L}_{FairPunt}$ ($\mathcal{L}_{FP}$) is:
\begin{equation}
\begin{aligned}
\mathcal{L}_{FP}(Y, A, (P, N, I)) = &-\bigg[\sum_i Y_i \log{P_i} + (1 - Y_i) \log{N_i} - \gamma\log{I_i}\bigg] \\
&+ \alpha (DI_{reg}(Y, A, P) + DI_{reg}(Y, A, N))
\end{aligned}
\end{equation}

Using hard thresholds simply restricts $P, I, N \in \{0, 1\}^3$, meaning that exactly one of $P, I, N$ will be 1, and the others 0. The regularized loss function with hard thresholds would be
\begin{equation} \label{disc_idk_fair_loss}
\begin{aligned}
% L = &(\sum_i Y_i \log{P_i} + (1 - Y_i) \log{N_i} + \gamma(\log{I_i})) \\
% &+ \alpha (DI_{reg}(Y, A, P_i) + DI_{reg}(Y, A, N_i))
\mathcal{L}_{FP}^{H}(Y, A, (P, N, I)) = &-\bigg[\sum_i \mathbbm{1}[Y_i == P_i] + \mathbbm{1}[(1 - Y_i) == N_i] - \gamma I_i \bigg]\\
&+ \alpha (DI(Y, A, P) + DI(Y, A, N))
\end{aligned}
\end{equation}
% \mathcal{L} = -\bigg[\sum_i \mathbbm{1}[Y_i == p_i]\bigg] + \alpha DI(Y, A, p); p \in \{0, 1\}

Note that we regularize the disparate impact for $P_i$ and $N_i$ separately. This was not necessary in the binary case, since these two probabilities would have always summed to 1.

\section{Learning to Defer} \label{learn_defer}

IDK classifiers come with a consequence - when a model punts, the prediction is made instead by some external, imperfect decision maker (DM). This external DM may be a human, a groups of humans, a biased software system, a company, or any sort of pipeline whose decisions are subject to their own strengths and weaknesses. It is essential that models which are intended to co-operate with external DMs can account for the DM's flaws, biases and idiosyncrasies. 

In the previous section, we discouraged IDK by adding a cost in the loss function. However, in many real world scenarios, after the model says punts, a decision must still be made. It is possible that, even if our model is very accurate and fair when it \textit{does} predict, that when taking into account the predictions made by the DM on the punted examples, the total set of predictions will not be. For instance, if the model punts on mostly cases where the DM is very inaccurate or very unfair, then the joint predictions made by the model-DM pair may be very poor, even though the model's predictions are fair and accurate.  Essentially, the model's uncertainty should not be the only factor in learning whether to predict. Rather, we must consider also whether the DM's prediction may be superior or inferior to the model's prediction.
\begin{figure}
\centering
\includegraphics[width=0.47\textwidth]{defer-learning-flow.pdf} \caption{Data flow within larger system containing an IDK classifier. When the model predicts, the system outputs the model's prediction; when the model defers (says IDK), the system outputs the decision-maker's (DM's) prediction.}
\label{defer-learning}
\end{figure}
We make the distinction between \textit{learning to punt} and \textit{learning to defer}. In learning to punt, the goal is absolute: the model's aim is to identify the examples where it has a low chance of being correct. In learning to defer, the goal is relative: the model's aim is to identify the examples where the DM's chance of being correct is much higher than its own.  In addition, since the DM-machine system makes the decisions jointly, knowledge of the DM during training allows the combined model to be jointly fair and accurate. We can think of learning to punt as \textit{DM-unaware learning}, and learning to defer as \textit{DM-aware learning}.

In this paper we make the assumption that there exist cases where the DM is more able to make an more informed decision than the machine, but the DM is not fair. This is an important real-world scenario: perhaps the DM is a judge who has more detailed information on repeat offenders, or a doctor who can conduct a suite of complex medical tests. We prefer the model to \textit{not} make a prediction in these cases, but rather to recognize that it is less qualified than the DM, and to defer to the DM. At test time, the model will operate in a pipeline fashion - either the model makes a prediction, or the model defers and the DM makes a prediction. In this way, we will obtain a prediction on every example.

%connect to AI safety?


\subsection{Models which Defer}

To learn a model which is jointly fair with the DM, we need to conduct DM-aware learning: that is, we must take the DM into account during training. We can modify the model presented in Section \ref{ternary_class} to take an extra input: the DM's scores on every case in the training set. Then we can adjust the loss function to reflect the reality -- that when the model predicts IDK, we don't just pay some constant cost. Rather, our cost for predicting depends on the DM's output -- if the DM is correct, our IDK cost should be low; if the DM is incorrect, our IDK cost should be high.

We draw inspiration from mixture-of-experts \citep{jacobs1991adaptive}. We can interpret $ I_i \in [0, 1]$ from the ordinal regression (Eq. \ref{ordreg}) to be a mixing parameter between the machine and the DM. Let $\pi_i = I_i$. Then, $\hat{\pi_i} \sim Bern(\pi_i)$ is a Bernoulli variable which indicates who should make the prediction on example $i$. If $\hat{\pi_i} = 1$, the human predicts; if $\hat{\pi_i} = 0$, the machine predicts. So for high values of $\pi_i$, the model is very uncertain and prefers to defer; for low values of $\pi_i$, the model is confident in its own prediction, i.e.,
\begin{equation}
\begin{aligned}
\hat{Y}_i = \hat{\pi_i} \tilde{Y}_i + (1 - \hat{\pi_i}) p_i\\
\pi_i \in \{0, 1\}; \hat{Y}_i, \tilde{Y}_i, p_i \in [0, 1]
\end{aligned}
\end{equation}
where $\tilde{Y}_i$ is the DM's output on example $i$, and $p_i$ is a ordinal regression's prediction, independent of uncertainty (Eq. \ref{defn_p}).
We can then define our loss function ($\mathcal{L}_{Defer}$, or $\mathcal{L}_{D}$, with soft thresholds) as an expectation over these Bernoulli variables $\hat{\pi_i}$ using $\hat{Y}$ as defined above:
\begin{equation} \label{expected_loss_fn}
\begin{aligned}
\mathcal{L}_{D}(Y, A, &\hat{Y}) = \mathds{E}_{\hat{\pi}} \mathcal{L}(Y, A, \hat{Y})\\
=& \mathds{E}_{\hat{\pi}} \bigg[-\sum_i \big[Y_i \log{\hat{Y}_i} + (1 - Y_i) \log({1 - \hat{Y}_i}) - \gamma\log{\pi_i} \big]\\
& + \alpha DI_{reg}(Y, A, \hat{Y})\bigg]
\end{aligned}
\end{equation}

Note that the model is not learning the DM scores $\tilde{Y}$ -- rather, it takes them as input. With hard thresholds, $\hat{\pi} = \pi \in \{0, 1\}$, and we can modify this expression analogously to the previous section, in Eq. \ref{disc_idk_fair_loss}. When we optimize this expression, we are jointly optimizing the loss function incurred by the model and the DM, taking into consideration the model's uncertainty and the DM's own inaccuracies and biases. More details are given in the Appendix about how this expected value is calculated.

\section{Results}
\subsection{Experimental Setup}
In order to evaluate our models, we need to measure three quantities: classification error rate, disparate impact, and deferral rate. Due to a lack of data on real decision makers, we train an independent, automated model to simulate the predictions made by an external DM. This DM is trained on a version of the dataset with extra attributes, simulating the extra knowledge that the DM may have. Therefore, the DM has a lower error rate than the IDK model does. However, the DM is \textit{not} trained to be fair. When our model outputs IDK we take the output of the DM instead, simulating real-world situations where a decision must always be made - even when the model is unsure (see Figure \ref{defer-learning}.  The aim is to defer to the DM as few times as possible, while achieving low joint error rate and disparate impact.

First, we describe our data and training procedure. Then we show evidence that using a punting IDK model and fairness regularization (jointly or separately) can both provide improvements in fairness and/or accuracy. Finally, we demonstrate the advantage of learning to defer - we show that models which have learned to defer improve in both accuracy and disparate impact.

\subsection{Datasets and Experiment Details}

We show results on two datasets. The first is the COMPAS recidivism dataset, made available by ProPublica \citep{kirchner_machine_2016}  \footnote{downloaded from https://github.com/propublica/compas-analysis}. This dataset concerns recidivism: whether or not a criminal defendant will commit a crime while on bail. The goal is to predict whether or not the person will recidivate, and the sensitive variable is race (split into black and non-black). We used information about counts of prior charges, charge degree, sex, age, and charge type (e.g. robbery, drug possession). We provide one extra bit of information to our DM - whether or not the defendant \textit{violently} recidivated. This clearly delineates between two groups in the data - one where the DM knows the correct answer (those who violently recidivated) and one where the DM has no extra information (those who did not recidivate, and those who recidivated non-violently). This simulates a real-world scenario where a DM, unbeknownst to the model, may have extra information on a subset of the data. The simulated DM had a 24\% error rate, better than the baseline model's 29\% error rate. We split the dataset into 7718 training examples and 3309 test examples.

The second dataset is the Heritage Health dataset\footnote{Downloaded from https://www.kaggle.com/c/hhp}. This dataset concerns health and hospitalization, particularly with respect to insurance. For this dataset, we chose the goal of predicting the Charlson Index, a comorbidity indicator, related to someone's chances of death in the next several years. We binarize the Charlson Index of a patient as 0/greater than 0. We take the sensitive variable to be age and binarize by over/under 70 years old. This dataset contains information on sex, age, lab test, prescription, and claim details. The extra information available to the DM is the primary condition group of the patient (given in the form of a code e.g. 'SEIZURE', 'STROKE', 'PNEUM'). Again, this simulates the situation where a DM may have extra information on the patient's health that the algorithm does not have access to. The simulated DM had a 16\% error rate, better than the baseline model's 21\% error rate.  We split the dataset into 46769 training examples and 20044 test examples.

We trained all models using a one-layer fully connected neural network with a logistic or ordinal regression on the output, where appropriate. We used 5 sigmoid hidden units for COMPAS and 20 sigmoid hidden units for health. We used ADAM \citep{kingma2014adam} for gradient descent. We split the training data into 80\% training, 20\% validation, and stopped training after 50 consecutive epochs without achieving a new minimum loss on the validation set.

In the ordinal regression model, we trained with soft thresholds since we needed the model to be differentiable end to end. In the post-hoc model, we searched threshold space in a manner which did not require differentiability, so we used hard thresholds. This is equivalent to an ordinal regression which produces one-hot vectors i.e. $P, I, N \in \{0, 1\}$. See the Appendix for extra details on both of these cases.

\subsection{Displaying the Models' Performance}

All of the models we examine here contain a number of hyperparameters, such as the tradeoff coefficients ($\alpha, \gamma$) between the terms in the loss function used to train that model. As opposed to standard empirical plots, we show the results not only of a single model, with the hyperparameter setting that yielded the best results, but of several models, both to give a more complete picture and also to illustrate how these parameters mediate the tradeoff of model accuracy (Error on the x-axis) and fairness (DI on the y-axis). Each point on a plot is a median of 5 runs at a given hyperparameter setting, as the model performance also depends on initial random parameter settings.  We only show points on the so-called Pareto front of the results, i.e., those for which no other point had better error and DI. Finally, the results are all generalization results, solely based on test examples.

\subsection{Results: Learning to Punt} \label{res_idk}

% \begin{figure}
% \centering
% \begin{subfigure}{.6\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{ablation_compas_err_vs_di_bin_t__0_00_1_00__pareto_posthoc.pdf}
%   \caption{COMPAS dataset}
%   \label{ablation:compas-posthoc}
% \end{subfigure}%
% \begin{subfigure}{.6\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{ablation_health_err_vs_di_bin_t__0_00_1_00__pareto_posthoc.pdf}
%   \caption{Health dataset}
%   \label{ablation:health-posthoc}
% \end{subfigure}
% \caption{Comparing performance between IDK and binary models, with and without fairness term. Navigating trade-off between accuracy (x-axis) and DI (y-axis). Bottom left hand corner is optimal.}
% \label{ablation:posthoc}
% \end{figure}

\begin{figure}
\centering
\subcaptionbox{COMPAS dataset \label{ablation:compas-posthoc}}{%
  \includegraphics[width=0.48\textwidth]{ablation_compas_err_vs_di_bin_t__0_00_1_00__pareto_posthoc.pdf}%
  }\par\medskip     
\subcaptionbox{Health dataset \label{ablation:health-posthoc}}{%
  \includegraphics[width=0.48\textwidth]{ablation_health_err_vs_di_bin_t__0_00_1_00__pareto_posthoc.pdf}%
  }
\caption{Comparing performance between punting IDK and binary models, with and without fairness term. Navigating trade-off between accuracy (x-axis) and fairness (y-axis). Bottom left hand corner is optimal. The purple star is a baseline model, trained only to optimize accuracy; green squares is a model also optimizing fairness; the red diamond optimizes accuracy while allowing IDK; and blue circles are the full model with all three terms. Yellow star shows the second stage model DM alone.}
\label{ablation:posthoc}
\end{figure}

In Figure \ref{ablation:posthoc}, we compare punting models to binary models, with and without fairness regularization. These IDK models have \textit{not} learned to defer, i.e. they did not receive access to the DM scores during training (we discuss those in Section \ref{res_defer}). Since we evaluate the models on both error and DI, we need to look at the results along the trade-off at various hyperparameter settings. The results shown are post-hoc thresholding results, so there are 3 hyperparameters: $\alpha$ and $\gamma$ in thresholding (eq. \ref{expected_loss_fn}) and $\alpha$ from the first stage scores learned by a fair binary model (eq. \ref{cont_di_loss}). 

The results show that, on both datasets, the IDK models achieve a stronger combination of fairness and accuracy than the binary models. Graphically, we observe this by noting that the line of points representing IDK model results are closer to the lower left hand corner of the plot than the line of points representing binary model results. Some of this improvement is driven by the extra accuracy in the DM. However, it is still important to note that the model-DM combination achieves a more effective accuracy-fairness tradeoff than any of the three baselines: the accurate but unfair DM; the fair but inaccurate binary model with DI regularization; and the unfair and inaccurate unregularized binary model. Furthermore, working with a more accurate DM is an important practical concern, as discussed elsewhere in this paper. Learning to punt can therefore be a valuable tool for anyone who designs or oversees a many-part system - a simple first stage capable of expressing uncertainty can improve the fairness of a more accurate DM.

% Considering the possibility of a DM with higher accuracy is important for several reasons. Algorithms operate in many complex scenarios today, where expert opinion is necessary, or where not all information can either be made available or effectively digitized. For instance, it is possible that the DM has access to some sensitive information, which cannot be exposed to the algorithm for privacy/security reasons. There may be qualitative or highly complex variables at play, such as spoken testimony or a written report. The DM may be a computationally intensive model, which has access to technical resources that the IDK model does not. Therefore, we think the situation of a more accurate DM is a very valuable one to explore. Our results, which suggest that a simple model with the capacity to say IDK can improve the fairness of systems which rely on these DMs, are therefore highly relevant to a wide variety of applications.
\subsection{Results - Learning to Defer} \label{res_defer}
% \begin{figure}
% \centering
% \begin{subfigure}{.25\textwidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{compas_err_vs_di_bin_t__0_00_1_00__pareto_posthoc.pdf}
%   \caption{COMPAS dataset}
%   \label{comp:compas-posthoc}
% \end{subfigure}%
% \begin{subfigure}{.25\textwidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{health_err_vs_di_bin_t__0_00_1_00__pareto_posthoc.pdf}
%   \caption{Health dataset}
%   \label{comp:health-posthoc}
% \end{subfigure}
% \caption{Comparing model performance with and without DM score training (i.e. Section \ref{ternary_class} vs. Section \ref{learn_defer}, along tradeoff between accuracy (x-axis) and DI (y-axis). Bottom left hand corner is optimal. Pareto front shown: Each point is the median of 5 runs at a hyperparameter setting.}
% \label{comp:posthoc}
% \end{figure}

\begin{figure}
\centering
\subcaptionbox{COMPAS dataset \label{comp:compas-posthoc}}{%
  \includegraphics[width=0.48\textwidth]{compas_err_vs_di_bin_t__0_00_1_00__pareto_posthoc.pdf}%
  }\par\medskip     
\subcaptionbox{Health dataset \label{comp:health-posthoc}}{%
  \includegraphics[width=0.48\textwidth]{health_err_vs_di_bin_t__0_00_1_00__pareto_posthoc.pdf}%
  }
 \caption{Comparison of DM-aware and -unaware learning (i.e., Section \ref{ternary_class} vs. Section \ref{learn_defer}), along tradeoff between accuracy (x-axis) and DI (y-axis). Bottom left hand corner is optimal. Each point is the median of 5 runs at a hyperparameter setting. Most of the results are the same as in Figure 3; the new results here show the performance of a DM-aware model (defer-fair).}
\label{comp:posthoc}
\end{figure}

Figure \ref{res_defer} compares deferring models (DM-aware, Section \ref{learn_defer}) with punting models (DM-unaware, Section \ref{ternary_class}). Again, each point is the median of 5 runs at a hyperparameter setting, and we show the Pareto front for each model. These results demonstrate a clear win for learning to defer - we can achieve substantially better fairness/accuracy by training with awareness of the DM. This can be seen graphically by observing that the line of points representing the DM-aware model is closer to the lower left than the line of points representing the DM-unaware model.

This result improves upon the results in Section \ref{res_idk}, demonstrating more clearly that a model which can defer is a valuable piece in a decision-making system. Particularly if we have access to examples of past DM behavior, learning to defer provides an effective way to improve the fairness of the \textit{entire system}.

To conceptually differentiate between these two models, we can inspect the different roles IDK plays in their respective loss functions. In the DM-unaware IDK model, an punting is penalized at a constant rate, determined by $\gamma$. However, in the DM-aware model, deferring penalized in a way which is \textit{dependent on the output of the DM} on that example. We can interpret the DM-unaware model within the DM-aware framework, by considering the unaware model to be optimizing the expected joint loss function for a DM whose expected loss on any example is constant; such as an oracle, or perfectly random (see the Appendix for experimental results on this). Then, we can see any improvement by the DM-aware model as effective identification of the examples on which the expected loss of the DM is unusually high - in other words, identifying the inconsistencies or biases of the DM.

\subsection{Results: Learning to Defer, by Deferral Rate} \label{res_defer_idkrate}
\begin{figure*}[t]
\begin{subfigure}[b]{0.3\linewidth}
  \centering
  \includegraphics[width=1.1\linewidth]{compas_err_vs_di_bin_t__0_00_0_30__pareto_posthoc.pdf}
  \caption{COMPAS, Low Deferral Rate (0-30\%)}
  \label{ex0}
\end{subfigure}\hfill
\begin{subfigure}[b]{.3\linewidth}
  \centering
  \includegraphics[width=1.1\linewidth]{compas_err_vs_di_bin_t__0_30_0_70__pareto_posthoc.pdf}
  \caption{COMPAS, Med Deferral Rate (30-70\%)}
  \label{ex1}
\end{subfigure}\hfill
\begin{subfigure}[b]{.3\linewidth}
  \centering
  \includegraphics[width=1.1\linewidth]{compas_err_vs_di_bin_t__0_70_1_00__pareto_posthoc.pdf}
  \caption{COMPAS, High Deferral Rate (70-100\%)}
  \label{ex2}
\end{subfigure}\\
\begin{subfigure}[b]{.3\linewidth}
  \centering
  \includegraphics[width=1.1\linewidth]{health_err_vs_di_bin_t__0_00_0_20__pareto_posthoc.pdf}
  \caption{Health, Low Deferral Rate (0-20\%)}
  \label{ex3}
\end{subfigure}\hfill
\begin{subfigure}[b]{.3\linewidth}
  \centering
  \includegraphics[width=1.1\linewidth]{health_err_vs_di_bin_t__0_20_0_40__pareto_posthoc.pdf}
  \caption{Health, Med Deferral Rate (20-40\%)}
  \label{ex4}
\end{subfigure}\hfill
\begin{subfigure}[b]{.3\linewidth}
  \centering
  \includegraphics[width=1.1\linewidth]{health_err_vs_di_bin_t__0_40_1_00__pareto_posthoc.pdf}
  \caption{Health, High Deferral Rate (40-100\%)}
  \label{ex5}
\end{subfigure}
\caption{Comparison of DM-aware and -unaware learning. Split into 3 bins, low, medium, and high deferral rate for each dataset. Bins are different between datasets due to the differing distributions of deferral rate observed during hyperparameter search.}
\label{comp-by-bin:posthoc}
\end{figure*}
% \begin{figure}
% \centering
% \begin{subfigure}{.25\textwidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{compas_err_vs_di_bin_t__0_00_0_30__pareto_posthoc.pdf}
%   \label{comp:compas-posthoc-0.3}
%   \caption{COMPAS dataset, IDK\% 0-0.3}
% \end{subfigure}%
% \begin{subfigure}{.25\textwidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{health_err_vs_di_bin_t__0_00_0_20__pareto_posthoc.pdf}
%   \label{comp:health-posthoc-0.3}
%     \caption{Health dataset, IDK\% 0-0.2}
% \end{subfigure}
% \label{comp:posthoc-low}
% \end{figure}

% \begin{figure}
% \centering
% \begin{subfigure}{.25\textwidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{compas_err_vs_di_bin_t__0_30_0_70__pareto_posthoc.pdf}
%   \label{comp:compas-posthoc-0.7}
%   \caption{COMPAS dataset, IDK\% 0.3-0.7}
% \end{subfigure}%
% \begin{subfigure}{.25\textwidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{health_err_vs_di_bin_t__0_20_0_40__pareto_posthoc.pdf}
%   \label{comp:health-posthoc-0.7}
%     \caption{Health dataset, IDK\% 0.2-0.4}
% \end{subfigure}
% \label{comp:posthoc-med}
% \end{figure}

% \begin{figure}
% \centering
% \begin{subfigure}{.25\textwidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{compas_err_vs_di_bin_t__0_70_1_00__pareto_posthoc.pdf}
%   \caption{COMPAS dataset, IDK\% 0.7-1}
%   \label{comp:compas-posthoc-1}
% \end{subfigure}%
% \begin{subfigure}{.25\textwidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{health_err_vs_di_bin_t__0_40_1_00__pareto_posthoc.pdf}
%   \caption{Health dataset, IDK\% 0.4-1}
%   \label{comp:health-posthoc-1}
% \end{subfigure}
% \label{comp:posthoc-high}
% \caption{Comparing model performance with and without DM score training (i.e. Section \ref{ternary_class} vs. Section \ref{learn_defer}, along tradeoff between accuracy (x-axis) and DI (y-axis). Bottom left hand corner is optimal. Pareto front shown: Each point is the median of 5 runs at a hyperparameter setting. Models binned by deferral rates}
% \end{figure}
Models which rarely defer behave very differently from those which frequently defer. In Figure \ref{comp-by-bin:posthoc}, we break down the results from Section \ref{res_defer} by deferral (or punting) rate. First, we note that even for models with similar deferral rates, we see a similar fairness/accuracy win for the DM-aware models. Next, we can look separately at the low and high deferral rate models. We note that the benefit of DM-aware training is much larger for high deferral rate models. This suggests that the largest benefit of learning to defer comes from a win in fairness, rather than accuracy.


% which means the examples the model does not defer on are the ones to look further into.

\section{Conclusion}
In this work, we propose the idea of learning to defer. We connect two problems prevalent in machine learning: bias and non-transparency. A model which defers is more transparent, since it is capable of communicating its uncertainty. We propose a model which learns to defer fairly, and show that deferring models can more effectively navigate the accuracy-fairness tradeoff.

We also consider deferring models that are part of a decision pipeline. To this end, we provide a framework for evaluating deferring models by encorporating other decision makers output into learning. We give an algorithm for learning to defer in the context of a larger system. We show that through awareness of other decision makers in the pipeline, we can effectively train a deferring model to optimize the performance of the pipeline as a whole. 

This result has ramifications for many complex domains where automated models interact with other decision-making agents. A model with a low deferral rate could be used to cull a large pool of examples, with all deferrals requiring further examination. Conversely, a model with a high deferral rate can be thought of as flagging the most troublesome, incorrect, or biased decisions by a DM, with all non-deferrals requiring further investigation.

Automated models often operate within larger systems, with many moving parts. Through deferring, we show how models can learn to predict responsibly within their surrounding systems. Building models which can defer to more capable decision makers is an essential step towards fairer, more responsible machine learning.

% Bibliography
\bibliographystyle{ACM-Reference-Format}
\bibliography{fatconference}

\appendix
\section{Results: Binary Classification with Fair Regularization}
The results in Figures \ref{di_plots} and \ref{err_plots} roughly replicate the results from \citep{bechavod_learning_2017}, who also test on the COMPAS dataset. Their results are slightly different for two reasons: 1) we use a 1-layer NN and they use logistic regression; and 2) our training/test splits are different from theirs - we have more examples in our training set. However, the main takeaway is similar: regularization with a disparate impact term is a good way to reduce DI without making too many more errors.
\begin{figure}
\centering
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{compas_di_by_alpha.png}
  \caption{COMPAS dataset}
  \label{compas_di_alpha}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{health_di_by_alpha.png}
  \caption{Health dataset}
  \label{health_di_alpha}
\end{subfigure}
\caption{Relationship of DI to $\alpha$, the coefficient on the DI regularizer, 5 runs for each value of $\alpha$}
\label{di_plots}
\end{figure}
\begin{figure}
\centering
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{compas_err_by_alpha.png}
  \caption{COMPAS dataset}
  \label{compas_err_alpha}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{health_err_by_alpha.png}
  \caption{Health dataset}
  \label{health_err_alpha}
\end{subfigure}
\caption{Relationship of error rate to $\alpha$, the coefficient on the DI regularizer, 5 runs for each value of $\alpha$}
\label{err_plots}
\end{figure}

\section{Details on Optimization: Hard Thresholds}

We now explain the post-hoc threshold optimization search procedure we used. In theory, any procedure can work. Since it is a very small space (one dimension per threshold = 4 dimensions), we used a random search. We sampled 1000 combinations of thresholds, picked the thresholds which minimized the loss on one half of the test set, and evaluated these thresholds on the other half of the test set. We do this for several values of $\alpha, \gamma$ in thresholding, as well as several values of $\alpha$ for the original binary model.

We did not sample thresholds from the [0, 1] interval uniformly. Rather we used the following procedure. We sampled our lower thresholds from the scores in the training set which were below 0.5, and our upper thresholds from the scores in the training set which were above 0.5. Our sampling scheme was guided by two principles: this forced 0.5 to always be in the IDK region; and this allowed us to sample more thresholds where the scores were more dense. If only choosing one threshold per class, we sampled from the entire training set distribution, without dividing into above 0.5 and below 0.5.

This random search was significantly faster than grid search, and no less effective. It was also faster and more effective than gradient-based optimization methods for thresholds - the loss landscape seemed to have many local minima.

\section{Details on Training with Expected Loss: Soft Thresholds}
%soft thresholds - form of exp squared disparate impact
We go into more detail regarding the regularization term for expected disparate impact in Equation \ref{expected_loss_fn}. When using soft thresholds, it is not trivial to calculate the expected disparate impact regularizer:
\begin{equation}
\begin{aligned}
DI_{exp}(Y, A, \hat{Y}) &= \mathds{E}_{\hat{\pi}} DI_{reg}(Y, A, \hat{Y})\\
&= \mathds{E}_{\hat{\pi}}\frac{1}{2} (DI_{reg,Y=0}(Y, A, p) + DI_{reg,Y=1}(Y, A, p))
% DI_{reg,Y=0}(Y, A, p) &= | E(p_i | A = 0, Y = 0) - E(p_i | A = 1, Y = 0) |\\
% DI_{reg,Y=1}(Y, A, p) &= | E(1 - p_i | A = 0, Y = 1) - E(1 - p_i| A = 1, Y = 1) |\\
% DI_{reg}(Y, A, p) &= \frac{1}{2} (DI_{reg,Y=0}(Y, A, p) + DI_{reg,Y=1}(Y, A, p))
\end{aligned}
\end{equation}
due to the difficulties involved in taking the expected value of an absolute value. We instead chose to calculate a version of the regularizer with squared underlying terms:
\begin{equation}
\begin{aligned}
DI_{soft}(Y, A, \hat{Y}) &= \mathds{E}_{\hat{\pi}}\frac{1}{2} (DI_{reg,Y=0}(Y, A, \hat{Y})^2 + DI_{reg,Y=1}(Y, A, \hat{Y})^2)\\
&= \mathds{E}_{\hat{\pi}} (E(\hat{Y}_i | A = 0, Y = 0) - E(\hat{Y}_i | A = 1, Y = 0))^2 \\
&+ \mathds{E}_{\hat{\pi}}(E(1 - \hat{Y}_i | A = 0, Y = 1) - E(1 - \hat{Y}_i| A = 1, Y = 1))^2\\
= &\mathds{E}_{\hat{\pi}}\bigg(\frac{\sum_i^n(1 - Y_i)(1 - A_i)\hat{Y}_i}{\sum_i^n (1 - Y_i)(1 - A_i)} - \frac{\sum_i^n (1 - Y_i)A_i\hat{Y}_i}{\sum_i^n (1 - Y_i)A_i}\bigg)^2 \\
+ &\mathds{E}_{\hat{\pi}}\bigg(\frac{\sum_i^n Y_i(1 - A_i)(1 - \hat{Y}_i)}{\sum_i^n Y_i(1 - A_i)}- \frac{\sum_i^n Y_iA_i (1 - \hat{Y}_i)}{\sum_i^n Y_iA_i}\bigg)^2\\
\end{aligned}
\end{equation}
Then, we can expand $\hat{Y}_i$ as
\begin{equation}
\begin{aligned}
\hat{Y}_i = \hat{\pi_i} \tilde{Y}_i + (1 - \hat{\pi_i}) p_i
\end{aligned}
\end{equation}
where $\tilde{Y}_i \in [0, 1]$ and $S(x_i) \in [0, 1]$ are the DM and machine predictions respectively. For brevity we will not show the rest of the calculation, but with some algebra we can obtain a closed form expression for $DI_{soft}(Y, A, \hat{Y})$ in terms of $Y, A, \tilde{Y}$ and $S$.
% Let $A_aY_y = \sum_i^n \mathbbm{1}{[Y_i = y, A_i = a]}$.
% \begin{equation}
% \begin{aligned}
% &= \bigg(\frac{\sum_i^n \mathbbm{1}{[Y_i = 0, A_i = 0]}\hat{Y}_i}{A_0Y_0} - \frac{\sum_i^n \mathbbm{1}{[Y_i = 0, A_i = 1]}\hat{Y}_i}{A_1Y_0}\bigg)^2 \\
% &+ \bigg(\frac{\sum_i^n \mathbbm{1}{[Y_i = 1, A_i = 0]}(1 - \hat{Y}_i)}{A_0Y_1} - \frac{\sum_i^n \mathbbm{1}{[Y_i = 1, A_i = 1]} (1 - \hat{Y}_i)}{A_1Y_1}\bigg)^2\\
% &= \bigg(\frac{\sum_i^n \mathbbm{1}{[Y_i = 0, A_i = 0]}\hat{Y}_i}{A_0Y_0} - \frac{\sum_i^n \mathbbm{1}{[Y_i = 0, A_i = 1]}\hat{Y}_i}{A_1Y_0}\bigg)^2 \\
% &+ \bigg(\frac{\sum_i^n \mathbbm{1}{[Y_i = 1, A_i = 0]}(1 - \hat{Y}_i)}{A_0Y_1} - \frac{\sum_i^n \mathbbm{1}{[Y_i = 1, A_i = 1]} (1 - \hat{Y}_i)}{A_1Y_1}\bigg)^2\\
% \end{aligned}
% \end{equation}

\section{Comparison of Oracle Training to IDK DM-Unaware}
\begin{figure}
\centering
\subcaptionbox{COMPAS dataset \label{oracle:compas-posthoc}}{%
  \includegraphics[width=0.4\textwidth]{compas_err_vs_di_bin_t__0_00_1_00__pareto_posthoc_nojoint.pdf}%
  }\par\medskip     
\subcaptionbox{Health dataset \label{oracle:health-posthoc}}{%
  \includegraphics[width=0.4\textwidth]{health_err_vs_di_bin_t__0_00_1_00__pareto_posthoc_nojoint.pdf}%
  }
 \caption{Comparing model performance between expected loss training with oracle as DM to IDK training unaware of DM. At test time, same DM is used.}
\label{oracle:posthoc}
\end{figure}

In Section \ref{res_defer}, we discuss that DM-unaware IDK training is similar to DM-aware training, except with a training DM who treats all examples similarly, in some sense. Here we show experimental evidence. The plots in Figure \ref{oracle:posthoc} compare these two models: DM-unaware, and DM-aware with an oracle at training time, and the standard DM at test time. We can see that these models trade off between error rate and DI in almost an identical manner.

%soft thresholds - form of exp squared disparate impact
